Controlling Mixing Inside a Droplet by Time Dependent Rigid-body Rotation

The use of microscopic discrete fluid volumes (i.e., droplets) as microreactors for digital microfluidic applications often requires mixing enhancement and control within droplets. In this work, we consider a translating spherical liquid droplet to which we impose a time periodic rigid-body rotation which we model using the superposition of a Hill vortex and an unsteady rigid body rotation. This perturbation in the form of a rotation not only creates a three-dimensional chaotic mixing region, which operates through the stretching and folding of material lines, but also offers the possibility of controlling both the size and the location of the mixing. Such a control is achieved by judiciously adjusting the three parameters that characterize the rotation, i.e., the rotation amplitude, frequency and orientation of the rotation. As the size of the mixing region is increased, complete mixing within the drop is obtained.

==> asme2e.cls1.3 <==
% ASME DOCUMENT CLASS - asme.cls
% 	for LaTeX version 2e - 2/14/01
%
% WARNING: This is an unauthorized class file. It has not been thoroughly
% tested so it probably still has bugs. I'll do my best to fix them when 
% found.
%
% ---------------------------------------------------------------------------
%   filename:      asme.cls
%   version:       2.1
%   date:          6/29/01
%   ported by:     Kenneth Sprott
%   address:       Department of Mechanical Engineering
%		   University of California, Davis
%		   Davis, California 95616
%   e-mail:        kssprott@ucdavis.edu
%   description:   This is a new version of the asme2e class file v1.0.
%		   New features in this file include:
%		   1. Eliminating the pifont package from the file.
%		      It was not required and had caused some problems.
%		   2. Fixed the font size definitions.  It is now possible
%		      to use 10, 11, and 12pt font.  The old size definition
%		      was incorrect and the default 12pt was actually 10pt.
%		      The default is now 10pt.
%		   3. Add support for the new reference format required by
%		      ASME. This requires the use of Bibtex.
%                  4. Eliminate the subfigure code held over from the original 
%                     ASME style file. Usepackage subfigure instead.
%                  5. Add cleanhead option to eliminate the banner on the title
%                     page.
%                  6. Add cleanfoot option to eliminate the copyright on each 
%                     footer.
%   usage:         \documentclass[options]{asme}
% ---------------------------------------------------------------------------

\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{asme2e}[2001/2/14 v2.0 Standard LaTeX document class]

\RequirePackage{ifthen}
\RequirePackage{times}      % Loads the Times-Roman Fonts
\RequirePackage{mathptm}    % Loads the Times-Roman Math Fonts



\newboolean{@titlepage}
\newcommand\@ptsize{}
\newboolean{@cleanfoot}
\newboolean{@cleanhead}

% -------------------------------------------------------
%                   Options
% -------------------------------------------------------

\DeclareOption{twoside}{\@twosidetrue \@mparswitchtrue}
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}
\DeclareOption{draft}{\setlength\overfullrule{5pt}}
\DeclareOption{final}{\setlength\overfullrule{0pt}}
\DeclareOption{titlepage}{\@titlepagetrue}
\DeclareOption{notitlepage}{\@titlepagefalse}
\DeclareOption{twocolumn}{\@twocolumntrue}
\DeclareOption{cleanfoot}{\@cleanfoottrue}
\DeclareOption{cleanhead}{\@cleanheadtrue}
\DeclareOption{10pt}{\renewcommand\@ptsize{0}} % Corresponds to 10pt font
\DeclareOption{11pt}{\renewcommand\@ptsize{1}} % Corresponds to 11pt font
\DeclareOption{12pt}{\renewcommand\@ptsize{2}} % Corresponds to 12pt font

\ExecuteOptions{oneside,onecolumn,10pt,final}
\ProcessOptions


\newcommand\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
\newcommand\currenttime{\minute\time\hour\minute\divide\hour60
\the\hour:\multiply\hour60\advance\minute-\hour\the\minute}



% ------------------------------------------------------
%                Font and Size Definitions 
% ------------------------------------------------------

\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand{\baselinestretch}{1}

% These next conditional statements set up the font size definitions
% for either 10, 11, or 12 pt font.  The default is 10pt.

\ifthenelse{\@ptsize = 0}{
\typeout{Ten Point}
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xpt{12}%
   \abovedisplayskip 18\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \abovedisplayskip 
   \belowdisplayshortskip \abovedisplayskip 
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@ixpt{11}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \belowdisplayskip \abovedisplayskip}
\newcommand\footnotesize{%
   \@setfontsize\footnotesize\@viiipt{10}
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus\p@
   \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 3\p@ \@plus\p@ \@minus\p@
               \parsep \z@ 
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip}
\newcommand\scriptsize{\@setfontsize\scriptsize\@viipt{8}}
\newcommand\tiny{\@setfontsize\tiny\@vpt{6}}
\newcommand\large{\@setfontsize\large\@xiipt{14}}
\newcommand\Large{\@setfontsize\Large\@xivpt{18}}
\newcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\newcommand\huge{\@setfontsize\huge\@xxpt{25}}
\newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}


\def\@listI{\leftmargin\leftmargini
            \parsep 4\p@ \@plus2\p@ \@minus\p@
            \topsep 8\p@ \@plus2\p@ \@minus4\p@
            \itemsep4\p@ \@plus2\p@ \@minus\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    4\p@ \@plus2\p@ \@minus\p@
              \parsep    2\p@ \@plus\p@  \@minus\p@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    2\p@ \@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}
}{}

\ifthenelse{\@ptsize = 1}{
\typeout{Eleven Point}
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xipt{13.6}%
   \abovedisplayskip 19\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@xpt\@xiipt
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 6\p@ \@plus2\p@ \@minus2\p@
               \parsep 3\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\footnotesize{%
   \@setfontsize\footnotesize\@ixpt{11}%
   \abovedisplayskip 8\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep \z@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{9.5}}
\newcommand\tiny{\@setfontsize\tiny\@vipt\@viipt}
\newcommand\large{\@setfontsize\large\@xiipt{14}}
\newcommand\Large{\@setfontsize\Large\@xivpt{18}}
\newcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\newcommand\huge{\@setfontsize\huge\@xxpt{25}}
\newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
\def\@listI{\leftmargin\leftmargini
            \parsep 4.5\p@ \@plus2\p@ \@minus\p@
            \topsep 9\p@   \@plus3\p@ \@minus5\p@
            \itemsep4.5\p@ \@plus2\p@ \@minus\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    4.5\p@ \@plus2\p@ \@minus\p@
              \parsep    2\p@   \@plus\p@  \@minus\p@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    2\p@ \@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}
}{}

\ifthenelse{\@ptsize = 2}{
\typeout{Twelve Point}
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xiipt{14.5}%
   \abovedisplayskip 20\p@ \@plus3\p@ \@minus7\p@
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@xipt{13.6}%
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 9\p@ \@plus3\p@ \@minus5\p@
               \parsep 4.5\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\footnotesize{%
   \@setfontsize\footnotesize\@xpt\@xiipt
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 6\p@ \@plus2\p@ \@minus2\p@
               \parsep 3\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{9.5}}
\newcommand\tiny{\@setfontsize\tiny\@vipt\@viipt}
\newcommand\large{\@setfontsize\large\@xivpt{18}}
\newcommand\Large{\@setfontsize\Large\@xviipt{22}}
\newcommand\LARGE{\@setfontsize\LARGE\@xxpt{25}}
\newcommand\huge{\@setfontsize\huge\@xxvpt{30}}
\let\Huge=\huge
\def\@listI{\leftmargin\leftmargini
            \parsep 5\p@  \@plus2.5\p@ \@minus\p@
            \topsep 10\p@ \@plus4\p@   \@minus6\p@
            \itemsep5\p@  \@plus2.5\p@ \@minus\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    5\p@   \@plus2.5\p@ \@minus\p@
              \parsep    2.5\p@ \@plus\p@    \@minus\p@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    2.5\p@\@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}
}{}



% These are specific fonts used in the file.

\DeclareFixedFont{\ninsfb}{OT1}{phv}{b}{n}{9}
\DeclareFixedFont{\ninsf}{OT1}{phv}{m}{n}{9}
\DeclareFixedFont{\egtsf}{OT1}{phv}{m}{n}{8}
\DeclareFixedFont{\egtsfb}{OT1}{phv}{b}{n}{8}
\DeclareFixedFont{\sevsf}{OT1}{phv}{m}{n}{7}
\DeclareFixedFont{\bannerfnt}{OT1}{phv}{b}{n}{10}
\DeclareFixedFont{\pnumfnt}{OT1}{phv}{b}{n}{18}
\DeclareFixedFont{\twlsfb}{OT1}{phv}{b}{n}{12}
\DeclareFixedFont{\tensfb}{OT1}{phv}{b}{n}{10}
\DeclareFixedFont{\tensf}{OT1}{phv}{m}{n}{10}

\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch{\relax}{\mathcal}}
\DeclareRobustCommand*\mit{\@fontswitch{\relax}{\mathnormal}}

\DeclareFontFamily{OT1}{msbm}{}
\DeclareFontShape{OT1}{msbm}{m}{n}{<5> <6> <7> <8> <9> <10> gen * msbm }{}

\newcommand\bb{\fontfamily{msbm}\selectfont}
\newcommand\bi{\fontseries{bc}\fontshape{it}\selectfont}

% -----------------------------------------------------------
%                 Page Layout
% -----------------------------------------------------------

\setlength{\paperheight}{11in}
\setlength{\paperwidth}{8.5in}
\setlength{\oddsidemargin}{48pt}
\setlength{\evensidemargin}{48pt}
\setlength{\topmargin}{2.0in}
\setlength{\marginparwidth}{0pt}
\setlength{\marginparsep}{11pt}
\setlength{\marginparpush}{5pt}
\setlength{\columnsep}{.375in}
\setlength{\columnseprule}{0pt}
\setlength{\headheight}{10pt}
\setlength{\headsep}{18pt}
\setlength{\topskip}{10pt}
\setlength{\footskip}{24pt}
\setlength{\textheight}{9.00in}
\advance\textheight by -\headheight
\advance\textheight by -\headsep
\setlength{\textwidth}{7.5in}
\setlength{\footnotesep}{6.65pt}
\setlength{\skip\footins}{9pt plus4pt minus 2pt}
\setlength{\floatsep}{18pt plus2pt minus2pt}
\setlength{\textfloatsep}{20pt plus4pt minus2pt}
\setlength{\intextsep}{24pt plus4pt minus2pt}
\setlength{\dblfloatsep}{12pt plus2pt minus2pt}
\setlength{\dbltextfloatsep}{20pt plus2pt minus4pt}
\setlength{\@fptop}{0pt plus 1fil}
\setlength{\@fpsep}{8pt plus 2fil}
\setlength{\@fpbot}{0pt plus 1fil}
\setlength{\@dblfptop}{0pt plus 1fil}
\setlength{\@dblfpsep}{8pt plus 2fil}
\setlength{\@dblfpbot}{0pt plus 1fil}
\setlength{\parskip}{0pt plus 1pt}
\setlength{\parindent}{.25in}
\setlength{\partopsep}{2pt plus 1pt minus 1pt}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty

\setlength{\leftmargini}{.25in}
\setlength{\leftmarginii}{22pt}
\setlength{\leftmarginiii}{18.7pt}
\setlength{\leftmarginiv}{17pt}
\setlength{\leftmarginv}{10pt}
\setlength{\leftmarginvi}{10pt}

% -------------------------------------------------------------------------
%                          Sections and Enumerate
% -------------------------------------------------------------------------

% Changes the enumerate environments

\setlength{\leftmargin}{\leftmargini}
\setlength{\labelsep}{5pt}
\setlength{\labelwidth}{\leftmargini}
\addtolength{\labelwidth}{-\labelsep}
\renewcommand{\@listI}{\leftmargin\leftmargini\parsep\z@
\topsep 6\p@ plus2\p@ minus1\p@\itemsep\z@}
\let\@listi\@listI
\@listi
\renewcommand{\@listii}{\setlength{\leftmargin}{\leftmarginii}
   \setlength{\labelwidth}{\leftmarginii}
   \addtolength{\labelwidth}{-\labelsep}
   \setlength{\topsep}{4\p@ plus2\p@ minus\p@}
   \setlength{\parsep}{\z@}
   \setlength{\itemsep}{\parsep}}
\renewcommand{\@listiii}{\setlength{\leftmargin}{\leftmarginiii}
    \setlength{\labelwidth}{\leftmarginiii}
    \addtolength{\labelwidth}{-\labelsep}
    \setlength{\topsep}{2\p@ plus\p@ minus\p@}
    \setlength{\parsep}{\z@}
    \setlength{\partopsep}{\p@ plus\z@ minus\p@}
    \setlength{\itemsep}{\parsep}}
\renewcommand{\@listiv}{\setlength{\leftmargin}{\leftmarginiv}
     \setlength{\labelwidth}{\leftmarginiv}
     \addtolength{\labelwidth}{-\labelsep}}
\renewcommand{\@listv}{\setlength{\leftmargin}{\leftmarginv}
     \setlength{\labelwidth}{\leftmarginv}
     \addtolength{\labelwidth}{-\labelsep}}
\renewcommand{\@listvi}{\setlength{\leftmargin}{\leftmarginvi}
     \setlength{\labelwidth}{\leftmarginvi}
     \addtolength{\labelwidth}{-\labelsep}}
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}


\newenvironment{verse}
               {\let\\=\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item[]}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item[]}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item[]}
               {\endlist}

\newenvironment{sequence}{      % Special enumerate environments for asme
    \renewcommand{\theenumi}{\alph{enumi}}
    \renewcommand{\labelenumi}{(\theenumi)}
    \begin{enumerate}}
    {\end{enumerate}}
\newenvironment{enumeroman}{
     \renewcommand{\theenumi}{\roman{enumi}}
     \renewcommand{\labelenumi}{(\theenumi)}
     \begin{enumerate}}
     {\end{enumerate}}
\newenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent-\leftmargin
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\newcommand*\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}

\renewcommand\theequation{\@arabic\c@equation}  % equation environment

\setlength\arraycolsep{1.5pt}  %Different from article class
\setlength\tabcolsep{6pt}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}

\renewcommand{\footnoterule}{    % This modifies the default footnote style
     \kern12\p@
     \hrule width.5in height.25pt
     \kern10\p@}

\long\def\@makefntext#1{\parindent 1em\noindent
    \hbox to1.8em{\hss$\m@th^{\@thefnmark}$}#1}

\def\@fnsymbol#1{\ifcase#1\or *\or \dagger\or \ddagger\or
  \Section\or \Paragraph\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi\relax}

% Title page definition

\newenvironment{titlepage}
    {%
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
        \@restonecolfalse\newpage
      \fi
      \thispagestyle{empty}%
      \if@compatibility
        \setcounter{page}{0}
      \else
        \setcounter{page}{1}%
      \fi}%
    {\if@restonecol\twocolumn \else \newpage \fi
      \setcounter{page}{1}%
    }


% Section Definitions

\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection .\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
\newcommand\part{\par
   \addvspace{4ex}%
   \@afterindentfalse
   \secdef\@part\@spart}

\def\@part[#1]#2{%
    \ifnum \c@secnumdepth >\m@ne
      \refstepcounter{part}%
      \addcontentsline{toc}{part}{\thepart\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >\m@ne
       \Large\bfseries \partname~\thepart
       \par\nobreak
     \fi
     \huge \bfseries #2%
     \markboth{}{}\par}%
    \nobreak
    \vskip 3ex
    \@afterheading}
\def\@spart#1{%
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \huge \bfseries #1\par}%
     \nobreak
     \vskip 3ex
     \@afterheading}
\def\@endpart{\vfil\newpage
              \if@twoside
                \hbox{}%
                \thispagestyle{empty}%
                \newpage
              \fi
              \if@tempswa
                \twocolumn
              \fi}

% This changes the section headings style

\newcommand{\section}{\@startsection {section}{1}{\z@}
                        {24pt plus3pt minus2pt}
                        {0.0001pt}
                        {\tensfb}}
\newcommand{\subsection}{\@startsection {subsection}{2}{\z@}
                           {18pt plus2pt minus1pt}
                           {0.0001pt}
                           {\tensfb}}
\newcommand{\subsubsection}{\@startsection {subsubsection}{3}{\parindent}
                           {18pt plus2pt minus1pt}
                           {-1em}
                           {\tensfb}}
\newcommand{\paragraph}{\@startsection {paragraph}{4}{\z@}
                          {12pt plus2pt minus1pt}
                          {-1em}
                          {\normalfont\normalsize\bfseries}}
\newcommand{\subparagraph}{\@startsection {subparagraph}{4}{\parindent}
                            {12pt plus2pt minus1pt}
                            {-1em}
                            {\normalfont\normalsize\bfseries}}

% -----------------------------------------------------------------------
%                         Table of Contents
% -----------------------------------------------------------------------

\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname
        \@mkboth{%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@part[2]{%
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries #1\hfil \hb@xt@\@pnumwidth{\hss #2}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\newcommand\listoffigures{%
    \section*{{List of Figures}
      \@mkboth{\MakeUppercase{List of Figures}}
              {\MakeUppercase{List of Figures}}}
    \@starttoc{lof}%
    }
\newcommand*\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
\newcommand\listoftables{%
    \section*{{List of Tables}
      \@mkboth{%
          \MakeUppercase{List of Tables}}
         {\MakeUppercase{List of Tables}}}
    \@starttoc{lot}%
    }
\let\l@table\l@figure

% ------------------------------------------------------------------------
%                         Tables and Figures
% ------------------------------------------------------------------------
\setcounter{topnumber}{4}         % These change the float placement 
\renewcommand{\topfraction}{.9}
\setcounter{bottomnumber}{4}
\renewcommand{\bottomfraction}{.9}
\setcounter{totalnumber}{4}
\renewcommand{\textfraction}{.1}
\renewcommand{\floatpagefraction}{.901}
\setcounter{dbltopnumber}{4}
\renewcommand{\dbltopfraction}{.9}
\renewcommand{\dblfloatpagefraction}{.91}         

\newcommand\figurename{Figure}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{APPENDIX}
\newcommand\refname{REFERENCES}
\newcommand\contentsname{CONTENTS}


\long\def\@makecaption#1#2{ % This remains the same from asme.sty
   \par\addvspace{6pt}{\tensf
   \setbox\@tempboxa\hbox{\egtsf#1.\quad#2}%
   \ifdim \wd\@tempboxa >\hsize
       {\egtsf#1.\quad\ignorespaces#2}\par
     \else
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
   \fi}} % \vskip4pt\global\c@subfigure0}
% Take out subfigure usepackage subfigure to achieve same result
%\newcounter{subfigure}
%\long\def\subcaption#1{%
%\global\advance\c@subfigure1
%   \setbox\@tempboxa\hbox{{\egtsfb (\alph{subfigure})\hskip.5em#1}}%
%   \ifdim \wd\@tempboxa >\hsize
%       {{\sffamily\fonsize{8}{\baselineskip}
%       (\alph{subfigure})\hskip.5em\ignorespaces#1\par}}
%     \else\hbox to\hsize{\hfil\box\@tempboxa\hfil}\fi\par\addvspace{6pt}}
\newbox\tempbox
\newcommand{\figurebox}[2]{%
            \dimen99=#2
            \divide\dimen99 by2
            \centerline{\vbox{\hrule\hbox to #1{\vrule\hfill\vbox to #2{\hbox to
            #1{\hfill{\vrule height\dimen99 width0pt{\hfill}}\hfill}\vfill}
            \vrule}\hrule}}}
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename~\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}{%
            \small
            \renewcommand{\arraystretch}{1.5}
            \@float{table}}
            {\end@float}
\newenvironment{table*}{%
            \small
            \renewcommand{\arraystretch}{1.5}
            \@dblfloat{table}}
            {\end@dblfloat}

\newcommand\x{@{\extracolsep{\hfill}}} % Command to control column space in
                                         % table environment.
% --------------------------------------------------------------------------
%                               Title Page
% --------------------------------------------------------------------------




\newcommand\@confshortname{}
\newcommand\@conffullname{}
\newcommand\@confdate{}
\newcommand\@confmonth{}
\newcommand\@confyear{}
\newcommand\@confcity{}
\newcommand\@confcountry{}
\newcommand\@papernum{}
\newcommand{\confshortname}[1]{\gdef\@confshortname{#1}}
\newcommand{\conffullname}[1]{\gdef\@conffullname{#1}}
\newcommand{\confdate}[1]{\gdef\@confdate{#1}}
\newcommand{\confmonth}[1]{\gdef\@confmonth{#1}}
\newcommand{\confyear}[1]{\gdef\@confyear{#1}}
\newcommand{\confcountry}[1]{\gdef\@confcountry{#1}}
\newcommand{\confcity}[1]{\gdef\@confcity{#1}}
\newcommand{\papernum}[1]{\gdef\@papernum{#1}}

\if@titlepage
  \newcommand{\maketitle}{\begin{titlepage}%
  \let\footnotesize\small
  \let\footnoterule\relax
  \null\vfil
  \vskip 60\p@
  \begin{center}%
    {\LARGE \@title \par}%
    \vskip 3em%
    {\large
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
      \vskip 1.5em%
    {\large \@date \par}%       % Set date in \large size.
  \end{center}\par
  \@thanks
  \vfil\null
  \end{titlepage}%
  \setcounter{footnote}{0}%
  \let\thanks\relax\let\maketitle\relax
  \gdef\@thanks{}\gdef\@author{}\gdef\@title{}}
\else
\newcommand{\maketitle}{\par
  \begingroup
    \renewcommand{\thefootnote}{\fnsymbol{footnote}}%
    \def\@makefnmark{\hbox to\z@{$\m@th^{\@thefnmark}$\hss}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hbox to1.8em{\hss$\m@th^{\@thefnmark}$}##1}%
    \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
      \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
    \thispagestyle{plain}\@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \let\thanks\relax
  \let\maketitle\relax\let\@maketitle\relax
  \gdef\@thanks{}\gdef\@author{}\gdef\@title{}}
\fi
 
\renewcommand\title[1]{\gdef\@title{\uppercase{#1}}}

\if@cleanhead
\def\@maketitle{%
  \newpage
  \null\vspace*{-26pt}
   \vbox{\hbox to \textwidth{\begin{tabular}{@{}c@{\hskip3pc}}
   \hbox to 46pt{\vbox to 46pt{\vss\hsize46pt\vss}}\end{tabular}\hss
  \vbox{\hsize37pc\scriptsize\sf\vskip\baselineskip%

  \vskip.5in}
  \hskip1pc}}
  \vskip.25in
  \vskip .25pc{\large\twlsfb
               \begin{center}\leftskip.5in plus1fill\rightskip\leftskip
               \@title\par\end{center}}
  \vskip2pc{\begin{center}\@author\par\end{center}}\vskip12pt}

\else

\def\@maketitle{%
  \newpage
  \null\vspace*{-26pt}             % Took out ASMElogo provision
   \vbox{\hbox to \textwidth{\begin{tabular}{@{}c@{\hskip3pc}}
   \hbox to 46pt{\vbox to 46pt{\vss\hsize46pt\vss}}\end{tabular}\hss
  \vbox{\hsize37pc\scriptsize\sf\vskip\baselineskip%
  \bannerfnt
  \hfill Proceedings of \@confshortname\par
  \hfill \@conffullname\par
  \hfill \@confmonth\ \@confdate, \@confyear, \@confcity, \@confcountry


  \vskip.5in
  \hfill {\pnumfnt\@papernum}}
  \hskip1pc}}
  \vskip.25in
  \vskip .25pc{\large\twlsfb
               \begin{center}\leftskip.5in plus1fill\rightskip\leftskip
               \@title\par\end{center}}
  \vskip2pc{\begin{center}\@author\par\end{center}}\vskip12pt}
\fi

\if@titlepage
  \newenvironment{abstract}{%
     \titlepage
     \null\vfil
     \begin{center}
        {\tensfb ABSTRACT}
        \@endparpenalty\@M
     \end{center}}
     {\par\vfil\null\endtitlepage}
\else
  \newenvironment{abstract}{%
     \if@twocolumn
        \normalsize\par\addvspace{12pt}\noindent
        {\tensfb ABSTRACT}\par
     \else
        \begin{center}
          {{\tensfb ABSTRACT}\vspace{-.5em}\vspace{\z@}}
        \end{center}
        \quotation
     \fi}
     {\if@twocolumn\else\endquotation\fi}
\fi 

% Get the multiple author set

\newcount\@authcnt
\newcount\@tmpcnt\@tmpcnt\z@

\def\@author{%
 \ifnum\@authcnt>7
  \ifnum\@tmpcnt<\@authcnt
   \global\advance\@tmpcnt1
   \leavevmode\hbox{\hss\csname @auth\romannumeral\the\@tmpcnt\endcsname\hss}%
   \quad
   \let\next\@author
  \else
   \let\next\relax
  \fi
 \else
  \ifnum\@tmpcnt<\@authcnt
   \global\advance\@tmpcnt1
   \ifnum\@tmpcnt=\@authcnt
    \expandafter\expandafter\expandafter\au@car\csname @auseq\romannumeral\the%
\@authcnt\endcsname\@nil
    \leavevmode\hbox to \@au@car{\hss\csname @auth\romannumeral\the\@tmpcnt%
\endcsname\hss}
   \else
    \expandafter\expandafter\expandafter\au@car\csname @auseq\romannumeral%
    \the\@authcnt\endcsname\@nil
    \leavevmode\hbox to \@au@car{\hss\csname @auth\romannumeral\the\@tmpcnt%
    \endcsname\hss}
   \fi
   \let\next\@author
  \else
   \let\next\relax
  \fi
 \fi
 \next}


\newcommand{\affiliation}[1]{\\ \tensf #1}

\def\@auseqi{{7.4in}}
\def\@auseqii{{3.45in}{3.45in}}
\def\@auseqiii{{2.4in}{2.4in}{2.4in}}
\def\@auseqiv{{3.45in}{3.45in}{3.45in}{3.45in}}
\def\@auseqv{{2.4in}{2.4in}{2.4in}{3.45in}{3.45in}}
\def\@auseqvi{{2.4in}{2.4in}{2.4in}{2.4in}{2.4in}{2.4in}}
\def\@auseqvii{{3.45in}{3.45in}{2.4in}{2.4in}{2.4in}{3.45in}{3.45in}}
\def\au@car#1#2\@nil{\gdef\@au@car{#1}}
\def\au@cdr#1#2\@nil{\expandafter\gdef\csname @auseq\romannumeral\the\@authcnt%
\endcsname{#2}}

\renewcommand{\author}[1]{%
    \global\advance\@authcnt1
    \expandafter\gdef\csname @auth\romannumeral\the\@authcnt\endcsname
    {\normalsize\sf\begin{tabular}[t]{@{}c@{}}\tensfb#1\\[20pt]
     \end{tabular}}}

% ---------------------------------------------------------------------------
%                           Bibliography 
% ---------------------------------------------------------------------------

\newcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}}

\newcommand\newblock{}
\newif\if@openbib
\@openbibfalse

% This generates the format for the bibliography enties. It is taken from
% the article class.

\newdimen\bibindent
\bibindent=1.5em
\newenvironment{thebibliography}[1]
     {\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \if@openbib
              \advance\leftmargin\bibindent
              \itemindent -\bibindent
              \listparindent \itemindent
              \parsep \z@
            \fi
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \if@openbib
        \renewcommand\newblock{\par}%
      \else
        \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
      \fi
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.=\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

% This code was borrowed from the cite.sty package.
%---------------------------------------------------------------------------
%     C I T E . S T Y
%
%     version 3.8  (Apr 1999)
%
%     Compressed, sorted lists of numerical citations: [11-16]
%     see also OVERCITE.STY and DRFTCITE.STY
%
%     Copyright (C) 1989-1999 by Donald Arseneau
%     These macros may be freely transmitted, reproduced, or modified
%     provided that this notice is left intact.
%
%     Instructions follow \endinput.
%  ------------------------------------
% First, ensure that some catcodes have the expected values


\edef\citenum{% to restore funny codes
  \catcode\string`\string ` \the\catcode\string`\`
  \catcode\string`\string ' \the\catcode\string`\'
  \catcode\string`\string = \the\catcode\string`\=
  \catcode\string`\string _ \the\catcode\string`\_
  \catcode\string`\string : \the\catcode\string`\:}
\catcode\string`\`12
\catcode`\'12
\catcode`\=12
\catcode`\_8
\catcode`\:12

%   Handle optional variations:  [verbose,nospace,space,nosort,noadjust],
%   \citeform,\citeleft,\citeright,\citemid,\citepunct,\citedash
%
%   Set defaults:

%   [ on the left.
\@ifundefined{citeleft}{\let\citeleft=[}{}

%   ] on the right:
\@ifundefined{citeright}{\let\citeright=]}{}

%   , (comma space) before note
\@ifundefined{citemid}{\def\citemid{,\penalty\@medpenalty\ }}{}

%   , (comma thin-space) between entries; [nospace] eliminates the space
\@ifundefined{citepunct}{
   \def\citepunct{,\penalty\@m\hskip.13emplus.1emminus.1em}%
 }{}

%   -- (endash) designating range of numbers:
% (using \hbox avoids easy \exhyphenpenalty breaks)
\@ifundefined{citedash}{\def\citedash{\hbox{--}\penalty\@m }}{}

%   Each number left as-is:
\@ifundefined{citeform}{\def\citeform{}}{}

%   Do not repeat warnings.  [verbose] reverses
\let\oc@verbo\relax

%----------------------
% \citen uses \@nocite to ignore spaces after commas, and write the aux file
% \citation. \citen then loops over the citation tags, using \@make@cite@list
% to make a sorted list of numbers.  Finally, \citen executes \@citelist to
% compress ranges of numbers and print the list. \citen can be used by itself
% to give citation numbers without the brackets and other formatting; e.g.,
% "See also ref.~\citen{junk}."
%
\edef\citen{\noexpand\protect \expandafter\noexpand\csname citen \endcsname}

\@namedef{citen }#1{%
\begingroup
\let\@safe@activesfalse\@empty
\@nocite{#1}% ignores spaces, writes to .aux file, returns #1 in \@no@sparg
\@tempcntb\m@ne    % \@tempcntb tracks highest number
\let\@h@ld\relax   % nothing held from list yet
\let\@citea\@empty % no punctuation preceding first
\let\@celt\delimiter % an unexpandable, but identifiable, token
\def\@cite@list{}% % empty list to start
\@for \@citeb:=\@no@sparg\do{\@make@cite@list}% make a sorted list of numbers
% After sorted citelist is made, execute it to compress citation ranges.
\@tempcnta\m@ne    % no previous number
\let\@celt\@compress@cite \@cite@list % output number list with compression
\@h@ld % output anything held over
\endgroup}

% For each citation, check if it is defined and if it is a number.
% if a number: insert it in the sorted \@cite@list
% otherwise: output it immediately.
%
\def\@make@cite@list{%
 \expandafter\let \expandafter\@B@citeB
          \csname b@\@citeb\@extra@b@citeb \endcsname
 \ifx\@B@citeB\relax % undefined: output ? and warning
    \@citea {\bf{?}}\let\@citea\citepunct \G@refundefinedtrue
    \@warning {Citation `\@citeb' on page \thepage\space undefined}%
    \oc@verbo \global\@namedef{b@\@citeb\@extra@b@citeb}{?}%
 \else %  defined               % remove previous line to repeat warnings
    \ifcat _\ifnum\z@<0\@B@citeB _\else A\fi % a positive number, put in list
       \@addto@cite@list
    \else % citation is not a number, output immediately
       \@citea \citeform{\@B@citeB}%
       \let\@citea\citepunct
 \fi\fi}

% Regular definition for adding entry to cite list, with sorting

\@ifundefined{@addto@cite@list}{% sort option either declared or defaulted
  \def\@addto@cite@list{\@tempcnta\@B@citeB \relax
     \ifnum \@tempcnta>\@tempcntb % new highest, add to end (efficiently)
        \edef\@cite@list{\@cite@list \@celt{\@B@citeB}}%
        \@tempcntb\@tempcnta
     \else % arbitrary number: insert appropriately
        \edef\@cite@list{\expandafter\@sort@celt \@cite@list \@gobble @}%
     \fi}
%
% \@sort@celt inserts number (\@tempcnta) into list of \@celt{num} (#1{#2})
% \@celt must not be expandable; list should end with two vanishing tokens.
%
  \def\@sort@celt#1#2{\ifx \@celt #1% parameters are \@celt {num}
       \ifnum #2<\@tempcnta % number goes later in list
          \@celt{#2}%
          \expandafter\expandafter\expandafter\@sort@celt % continue
       \else % number goes here
          \@celt{\number\@tempcnta}\@celt{#2}% stop comparing
    \fi\fi}
}% end sort option definitions
{}% nosort definition is done in options processing

% Check if each number follows previous and can be put in a range
%
\def\@compress@cite#1{%  % This is executed for each number
  \advance\@tempcnta\@ne % Now \@tempcnta is one more than the previous number
  \ifnum #1=\@tempcnta   % Number follows previous--hold on to it
     \ifx\@h@ld\relax    % first pair of successives
        \edef\@h@ld{\@citea \noexpand\citeform{#1}}%
     \else               % compressible list of successives
        \def\@h@ld{\citedash \citeform{#1}}%
     \fi
  \else   %  non-successor -- dump what's held and do this one
     \@h@ld \@citea \citeform{#1}\let\@h@ld\relax
  \fi \@tempcnta#1\let\@citea\citepunct
}

\edef\cite{\noexpand\protect\expandafter\noexpand\csname cite \endcsname}

\@namedef{cite }{\@ifnextchar [{\@tempswatrue\@citex}{\@tempswafalse\@citex[]}}

%  Make \@citex refer to \citen:
%
\def\@citex[#1]#2{\@cite{\citen{#2}}{#1}}%

%  Replacement for \@cite which defines the formatting normally done
%  around the citation list.  Minor changes can
%  be done by changing \citeleft, \citemid, and \citeright; but in other
%  cases it might be necessary to redefine the whole macro.
%
\def\@cite#1#2{\leavevmode \cite@adjust
  \citeleft{#1\if@tempswa \citemid #2\fi
  \spacefactor\@m % punctuation in note doesn't affect outside
  }\citeright}

%  Put a penalty before the citation, and adjust the spacing: if no space
%  already or if there is extra space due to some punctuation, then change
%  to one inter-word space.
%
\@ifundefined{cite@adjust}{\def\cite@adjust{%
  \@tempskipa\lastskip \edef\@tempa{\the\@tempskipa}\unskip
  \ifnum\lastpenalty=\z@ \penalty\@highpenalty \fi
  \ifx\@tempa\@zero@skip \spacefactor1001 \fi % if no space before, set flag
  \ifnum\spacefactor>\@m \ \else \hskip\@tempskipa \fi}}{}

\edef\@zero@skip{\the\z@skip}

% \nocite: This is changed to ignore *ALL* spaces and be robust.  The
% parameter list, with spaces removed, is `returned' in \@no@sparg, which
% is used by \citen.
%
\edef\nocite{\noexpand\protect\expandafter\noexpand\csname nocite \endcsname}

\@namedef{nocite }#1{\@bsphack \@nocite{#1}%
 \@for \@citeb:=\@no@sparg\do{\@ifundefined{b@\@citeb\@extra@b@citeb}%
    {\G@refundefinedtrue\@warning{Citation `\@citeb' undefined}%
    \oc@verbo \global\@namedef{b@\@citeb\@extra@b@citeb}{?}}{}}%
 \@esphack}

\def\@nocite#1{\xdef\@no@sparg{\@ignsp#1 \! }% remove *ALL* spaces
 \if@filesw \immediate\write\@auxout {\string\citation {\@no@sparg}}\fi}

% for ignoring *ALL* spaces in the input.  This presumes there are no
% \outer tokens and no \if-\fi constructs in the parameter.  Spaces inside
% braces are retained.
%
\def\@ignsp#1 {\ifx\!#1\@empty\else #1\expandafter\@ignsp\fi}

\let\nocitecount\relax  % in case \nocitecount was used for drftcite

\@ifundefined{@extra@b@citeb}{\def\@extra@b@citeb{}}{}
%  in case no fancy bib package (chapterbib) defines this

\@ifundefined{G@refundefinedtrue}{\let\G@refundefinedtrue\relax}{}

\citenum % execute restore-catcodes

% Aliases:
\let\citenum\citen
\let\citeonline\citen

% End of Cite.sty code.
%-------------------------------------------------------------------------


% ---------------------------------------------------------------------------
%                          Special ASME declarations
% --------------------------------------------------------------------------

% Nomenclature environment

\newbox\tempbox
\newenvironment{nomenclature}{%
   \newcommand\entry[2]{%
       \setbox\tempbox\hbox{##1.\quad}
       \hangindent\wd\tempbox\noindent{##1}\quad\ignorespaces##2\par}
       \section*{NOMENCLATURE}}{\par\addvspace{12pt}}

% Acknowledgement environment

\newenvironment{acknowledgment}{%
   \section*{ACKNOWLEDGMENT}}{\par\addvspace{12pt}}

% The following are the new theorem definitions


\AtEndOfClass{%
  \def\@begintheorem#1#2{\trivlist \item[\hskip \labelsep%
  {\tensfb #1\ #2.}]\it}
  \def\@opargbegintheorem#1#2#3{\trivlist
        \item[\hskip \labelsep%
  {\tensfb #1\ #2\ (#3).}]\it}
  \def\newtheorem{\@ifstar{\@newstheorem}{\@newtheorem}}
  \def\@newtheorem#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}
  \def\@newstheorem#1#2{\@namedef{#1*}
  {\@ifnextchar[{\@opargbeginstheorem{#2}}{\@beginstheorem{#2}}}%
  \@namedef{end#1*}{\@endtheorem}}
  \def\@beginstheorem#1{\trivlist \item[\hskip \labelsep%
  {\tensfb #1.}]\it}
  \def\@opargbeginstheorem#1[#2]{\trivlist\item[\hskip \labelsep%
  {\tensfb #1\ (#2).  }]\it}
%
  \def\proof{\@ifnextchar[{\@optargproof}{\@proof}}
  \def\@proof{\trivlist \item[\hskip \labelsep{\it Proof.}]}
  \def\@optargproof[#1]{\trivlist \item[\hskip \labelsep{\it #1.}]}
  \def\endproof{\endtrivlist}
  \def\qed{\vskip-\lastskip\vskip-\baselineskip\hbox to \hsize{\hfill$\Box$}} 
}


% -------------------------------------------------------------------------
%                 Header and Footer Definitions
% -------------------------------------------------------------------------

\if@twoside
  \def\ps@headings{%
      \let\@oddfoot\@empty\let\@evenfoot\@empty
      \def\@evenhead{\thepage\hfil\slshape\leftmark}%
      \def\@oddhead{{\slshape\rightmark}\hfil\thepage}%
      \let\@mkboth\markboth
    \def\sectionmark##1{%
      \markboth {\MakeUppercase{%
        \ifnum \c@secnumdepth >\z@
          \thesection\hskip 1em\relax
        \fi
        ##1}}{}}%
    \def\subsectionmark##1{%
      \markright {%
        \ifnum \c@secnumdepth >\@ne
          \thesubsection\quad
          \fi
          ##1}}}
\else
  \def\ps@headings{%
    \let\@oddfoot\@empty
    \def\@oddhead{{\slshape\rightmark}\hfil\thepage}%
    \let\@mkboth\markboth
    \def\sectionmark##1{%
      \markright {\MakeUppercase{%
        \ifnum \c@secnumdepth >\m@ne
          \thesection\quad
        \fi
        ##1}}}}
\fi

\if@cleanfoot
 \def\ps@myheadings{%
    \let\@mkboth\@gobbletwo
    \def\@oddfoot{\hfil\thepage\hfil}
    \def\@evenfoot{\hfil\thepage\hfil}
    \let\@oddhead\@empty\let\@evenhead\@empty
    \def\sectionmark##1{}
    \def\subsectionmark##1{}
    }
\def\ps@plain{\let\@mkboth\@gobbletwo
     \def\@oddhead{$\smash{\raise72pt\hbox%
                  {}}$\hfill}%
                  %{\scriptsize\today\qquad\currenttime}}$\hfill}%
     \def\@oddfoot{\reset@font\rm \hfil\thepage%
     \hfil}%
     \let\@evenhead\@oddhead\let\@evenfoot\@oddfoot}

\else
 \def\ps@myheadings{%
     \let\@mkboth\@gobbletwo
     \def\@oddfoot{\hskip1.55in\hfil\thepage\hfil Copyright\ \ \copyright\ \@confyear%
    ~by ASME}%
     \def\@evenfoot{\hskip1.55in\hfil\thepage\hfil Copyright\ \ \copyright\ \@confyear%
    ~by ASME}%

    \let\@oddhead\@empty
    \let\@evenhead\@empty
    \def\sectionmark##1{}
    \def\subsectionmark##1{}
    }
\def\ps@plain{\let\@mkboth\@gobbletwo
     \def\@oddhead{$\smash{\raise72pt\hbox%
                  {}}$\hfill}%
                  %{\scriptsize\today\qquad\currenttime}}$\hfill}%
     \def\@oddfoot{\reset@font\rm\hskip1.55in\hfil\thepage%
     \hfil Copyright\ \ \copyright\ \@confyear\ by ASME}%
     \let\@evenhead\@oddhead\let\@evenfoot\@oddfoot}

\fi

 
%\def\ps@myheadings{%
%    \let\@mkboth\@gobbletwo
%    \ifthenelse{\@cleanfoot = 1}{
%      \def\@oddfoot{\hskip1.55in\hfil\thepage}
%      \def\@evenfoot{\hskip1.55in\hfil\thepage}}
%      {\def\@oddfoot{\hskip1.55in\hfil\thepage\hfil Copyright\ \ \copyright\ \confyear%
%    ~by ASME}%
%      \def\@evenfoot{\hskip1.55in\hfil\thepage\hfil Copyright\ \ \copyright\ \confyear%
%    ~by ASME}%}
%
%\let\@oddhead\@empty
%\let\@evenhead\@empty
%%    \def\@evenhead{\hfil\sl\leftmark\hfil}%
%%    \def\@oddhead{\hfil\sl\rightmark\hfil}%
%    \def\sectionmark##1{}
%    \def\subsectionmark##1{}
%    }


\mark{{}{}}
%\def\ps@plain{\let\@mkboth\@gobbletwo
%     \def\@oddhead{$\smash{\raise72pt\hbox%
%                  {\scriptsize\today\qquad\currenttime}}$\hfill}%
%     \def\@oddfoot{\reset@font\rm\hskip1.55in\hfil\thepage%
%     \hfil Copyright\ \ \copyright\ \confyear\ by ASME}%
%     \let\@evenhead\@oddhead\let\@evenfoot\@oddfoot}

\newcount\minute\newcount\hour
\def\currenttime{\minute\time\hour\minute\divide\hour60
\the\hour:\multiply\hour60\advance\minute-\hour\the\minute}

\markboth{}{}
\ps@myheadings
\pagenumbering{arabic}
\if@twocolumn\twocolumn\sloppy\flushbottom\else\onecolumn\fi
\advance\hoffset-7pc
\advance\voffset-10pc
%
%
\endinput

% End of Class



